A Best-of-both-worlds Algorithm for Bandits with Delayed Feedback with Robustness to Excessive Delays

We propose a new best-of-both-worlds algorithm for bandits with variably delayed feedback. In contrast to prior work, which required prior knowledge of the maximal delay $d_{\mathrm{max}}$ and had a linear dependence of the regret on it, our algorithm can tolerate arbitrary excessive delays up to order $T$ (where $T$ is the time horizon). The algorithm is based on three technical innovations, which may all be of independent interest: (1) We introduce the first implicit exploration scheme that works in best-of-both-worlds setting. (2) We introduce the first control of distribution drift that does not rely on boundedness of delays. The control is based on the implicit exploration scheme and adaptive skipping of observations with excessive delays. (3) We introduce a procedure relating standard regret with drifted regret that does not rely on boundedness of delays. At the conceptual level, we demonstrate that complexity of best-of-both-worlds bandits with delayed feedback is characterized by the amount of information missing at the time of decision making (measured by the number of outstanding observations) rather than the time that the information is missing (measured by the delays).

==> evns.tex <==
% \theoremstyle{definition}
% \newtheorem*{examplex*}{Example}
% \newtheorem{examplex}{Example}
% \newenvironment{example*}
%   {\pushQED{\qed}\renewcommand{\qedsymbol}{$\square$}\begin{examplex*}}
%   {\popQED\end{examplex*}}
% \newenvironment{example}
%   {\pushQED{\qed}\renewcommand{\qedsymbol}{$\square$}\examplex}
%   {\popQED\endexamplex}
  
  
% \makeatletter
% \newcommand*{\algotitle}[2]{%
%   \stepcounter{algocf}%
%   \hypertarget{algocf.title.\theHalgocf}{}%
%   \NR@gettitle{#1}%
%   \label{#2}%
%   \addtocounter{algocf}{-1}%
% }
% \makeatother
% \theoremstyle{plain}
\newtheorem{claim}{Claim}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}



